On the Search for Feedback in Reinforcement Learning

The problem of Reinforcement Learning (RL) in an unknown nonlinear dynamical system is equivalent to the search for an optimal feedback law utilizing the simulations/ rollouts of the dynamical system. Most RL techniques search over a complex global nonlinear feedback parametrization making them suffer from high training times as well as variance. Instead, we advocate searching over a local feedback representation consisting of an open-loop sequence, and an associated optimal linear feedback law completely determined by the open-loop. We show that this alternate approach results in highly efficient training, the answers obtained are repeatable and hence reliable, and the resulting closed performance is superior to global state-of-the-art RL techniques. Finally, if we replan, whenever required, which is feasible due to the fast and reliable local solution, it allows us to recover global optimality of the resulting feedback law.

==> Decoupling_principle.tex <==
%\section{A Near-Optimal Decoupling Principle}
%\label{decoupling_principle}
\section{A NEAR OPTIMAL DECOUPLING PRINCIPLE}\label{sec3}
We outline a near-optimal decoupling principle in stochastic optimal control. 
We assume that the dynamics can be written in the control affine form 
$%$\begin{align} 
%\label{eq.0.1}
%\label{eq:dynamics1}
x_{t+1} = f(x_t) + g(x_t) u_t + \epsilon w_t, 
$%\end{align}
where $\epsilon < 1$ is a small parameter. We also assume that the instantaneous cost $c(\cdot, \cdot)$ has the following simple form, $c(x,u) = l(x) + \frac{1}{2} u'Ru.$
We emphasize that these assumptions,  quadratic  control cost and affine in control dynamics, are typically satisfied.

%With a slight abuse of notation, let $\pi^{*} = \pi = (\pi_{t})^{T}_{t=1}$ be the optimal control law given by \eqref{cost_sto_orig} according to the dynamics \eqref{eq.0.1} and instantaneous cost \eqref{eq:cost1}.   

\subsection{Characterization of the Performance of Feedback Policies}

Consider a noiseless  version of the system dynamics above. Denote the ``nominal'' state trajectory as $\bar{x}_{t}$ and the ``nominal'' control as $\bar{u}_{t}$ where $\bar{u}_{t} = \pi_{t}(\bar{x}_{t})$, and $\pi = (\pi_{t})^{T-1}_{t=1}$ is a given control policy. The resulting dynamics  without noise is given by $\bar{x}_{t+1} = f(\bar{x}_t) + g(\bar{x}_t) \bar{u}_t$.   

%Let the associated nominal incremental costs be denoted by $\bar{c}_t = l(\bar{x}_t) + \frac{1}{2} \bar{u}_t'R\bar{u}_t$, and the associated nominal terminal cost be denoted by $\bar{c}_T = c_T(\bar{x}_T)$. 

Assuming that $f(\cdot), g(\cdot)$ and $\pi_{t}(\cdot)$ are sufficiently smooth, we can expand the dynamics about the nominal trajectory. Denoting  $\delta x_t = x_t - \bar{x}_t, \delta u_t = u_t - \bar{u}_t$, we can express, 

\begin{align}
\label{eq2}
\delta x_{t+1} &= A_t \delta x_t + B_t \delta u_t + S_t(\delta x_t) + \epsilon w_t, \nonumber \\ %\label{eq2}
\delta u_{t} &=  K_t \delta x_t + \tilde{S}_t(\delta x_t), 
\end{align}

where $A_t = \frac{\partial f}{\partial x}|_{\bar{x}_t} + \frac{\partial g\bar{u}_t}{\partial x}|_{\bar{x}_t}$, $B_t = g(\bar{x}_t)$, $K_{t} = \frac{\partial \pi_{t}}{\partial x}|_{\bar{x}_t}$, and  $S_t(\cdot), \tilde{S}_t(\cdot)$ are second and higher order terms in the respective expansions. Similarly, we can linearize the instantaneous cost $c(x_{t}, u_{t})$ about the nominal values $(\bar{x}_{t}, \bar{u}_{t})$ as,
\begin{align}
\label{eq4}
c(x_t,u_t) &= {l}(\bar{x}_{t}) + L_t \delta x_t + H_t(\delta x_t) \nonumber\\ 
& + \frac{1}{2}\bar{u}_t'R\bar{u}_t +  \delta u_t'R\bar{u}_t + \frac{1}{2}\delta u_t'R\delta u_t,
\end{align}
\begin{align}
\label{eq5}
c_{T}(x_{T}) = {c}_{T}(\bar{x}_{T}) + C_T \delta x_T + H_T(\delta x_T),
\end{align}

where $L_t = \frac{\partial l}{\partial x}|_{\bar{x}_t}$, $C_T  = \frac{\partial c_T}{\partial x}|_{\bar{x}_t}$, and $H_t(\cdot)$ and $H_T(\cdot)$ are second and higher order terms in the respective expansions.

Using \eqref{eq2}, we can write the closed loop dynamics  of the trajectory $(\delta x_{t})^{T}_{t=1}$ as, 
\begin{align}
\label{eq6}
\delta x_{t+1} = \underbrace{(A_t+B_tK_t)}_{\bar{A}_t} \delta x_t + \underbrace{\{B_t\tilde{S}_t(\delta x_t) + S_t(\delta x_t)\}}_{\bar{S}_t(\delta x_t)} + \epsilon w_t, 
\end{align} 
where $\bar{A}_t$ represents the linear part of the closed loop systems and the term $\bar{S}_t(.)$ represents the second and higher order terms in the closed loop system. Similarly, the closed loop incremental cost given in  \eqref{eq4} can be expressed as
$%$\begin{align}
 %\label{eq7}
c(x_t,u_t) = \underbrace{\{{l}(\bar{x}_{t}) + \frac{1}{2}\bar{u}_t'R\bar{u}_t\}}_{\bar{c}_t} + \underbrace{[L_t + \bar{u}_t'RK_t]}_{\bar{C}_t} \delta x_t %\nonumber\\
+ \underbrace{\frac{1}{2}(K_t\delta x_t+\tilde{S}_t(\delta x_t))'R(K_t\delta x_t + \tilde{S}_t(\delta x_t)) + \bar{u}_t' R \tilde{S}_t(\delta x_t)}_{\bar{H}_t(\delta x_t)}. 
$%\end{align}

Therefore, the cumulative cost of any given closed loop trajectory $(x_{t}, u_{t})^{T}_{t=1}$  can be expressed as,
$%$\begin{align}
%\label{eq9a}
J^{\pi} = \sum^{T-1}_{t=1}c(x_{t}, u_{t} = \pi_{t}(x_{t})) + c_{T}(x_{T}) %\nonumber \\
=\sum_{t=1}^T \bar{c}_t + \sum_{t=1}^T \bar{C}_t \delta x_t + \sum_{t=1}^T \bar{H}_t(\delta x_t),
$%\end{align}
where $\bar{c}_{T} = c_{T}(\bar{x}_{T}),  \bar{C}_{T} = C_{T}$.

We first have the following critical result. 
\begin{lemma} 
\label{L1}
Given any sample path, the state perturbation equation 
% \[\delta x_{t+1} = \bar{A}_{t}  \delta x_{t} + \bar{S}_t(\delta x_t) + \epsilon w_t \]
$\delta x_{t+1} = \bar{A}_{t}  \delta x_{t} + \bar{S}_t(\delta x_t) + \epsilon w_t$
given in  \eqref{eq6} can be equivalently characterized  as
$\delta x_{t}  = \delta x_t^l + e_t, ~ \delta x_{t+1}^l = \bar{A}_t \delta x_t^l + \epsilon w_t$
where $e_t$ is an $O(\epsilon^2)$ function that depends on the entire noise history $\{w_0,w_1,\cdots w_t\}$ and $\delta x_t^l$ evolves according to the  linear closed loop system. Furthermore, $e_t = e_t^{(2)} + O(\epsilon^3)$, where $e_t^{(2)} = \bar{A}_{t-1} e_{t-1}^{(2)} + \delta x_t^{l'}\bar{S}_{t-1}^{(2)} \delta x_t^l$, $e_0^{(2)} = 0$, and $\bar{S}_t^{(2)}$ represents the Hessian corresponding to the Taylor series expansion of the function $\bar{S}_t(.)$. 
\end{lemma}

%Using  \eqref{eq:mod-pert-1} in  \eqref{eq.9a}, we can obtain the cumulative cost of any given closed loop trajectory as,
%\begin{align}
%J^{\pi} = \underbrace{\sum_{t=1}^T \bar{c}_t }_{\bar{J}^{\pi}} + \underbrace{\sum_{t=1}^T \bar{C}_t \delta x_t^l}_{\delta J_1^{\pi}} + %\nonumber\\
%\underbrace{\sum_{t=1}^T \bar{H}_t(\delta x_t) + \bar{C}_t \bar{\bar{S}}_t}_{\delta J_2^{\pi}}. \label{eq.9b}
%\end{align}
Next, we have the following result for the expansion of the cost to go function $J^{\pi}$.
\begin{lemma}
\label{L2}
Given any sample path, the cost-to-go under a policy can be expanded as: 
$J^{\pi}  = \underbrace{\sum_t \bar{c}_t}_{\bar{J}^{\pi}} + \underbrace{\sum_t \bar{C}_t \delta x_t^l}_{\delta J_1^{\pi}} + \underbrace{\sum_t \delta x_t^{l'}\bar{H}_t^{(2)} \delta x_t^l+ \bar{C}_t e_t^{(2)}}_{\delta J_2^{\pi}} + O(\epsilon^3),$
where $\bar{H}_t^{(2)}$ denotes the second order coefficient of the Taylor expansion of $\bar{H}_t(.)$.
\end{lemma}
Now, we have the following important result. 
\begin{proposition}  
\label{prop1} 
We have:$%$ \begin{align*}
\tilde{J}^{\pi} \equiv \mathbb{E}[J^{\pi} ] =  \bar{J}^{\pi} + O(\epsilon^2), %\\
 \text{Var}(J^{\pi}) =  \underbrace{\text{Var}(\delta J_{1}^{\pi})}_{O(\epsilon^{2})} +  O(\epsilon^4). 
 $%\end{align*}
 \end{proposition}
 All proofs can be found in the supplementary file.

A further consequence of the result above is the following. Suppose that given a policy $\pi_t(.)$, we only consider the linear part, i.e., the linear approximation $\pi_t^l(x_t) = \bar{u}_t + K_t\delta x_t$. According to Lemmas \ref{L1} and \ref{L2}, the $O(\epsilon^2)$ terms in the expansion of the cost of any sample path solely result from the linear closed loop system. Therefore, it follows that the sample path cost under the full policy $\pi_t(.)$ and the linear policy $\pi_t^l(.)$ agree up to the $\epsilon^2$ term. Therefore, it follows that $|E[J^{\pi}] - E[J^{\pi^l}]|  = O(\epsilon^4)$. We summarize this result in the following result:
\begin{proposition}
\label{prop2}
Let $\pi_t(.)$ be any given feedback policy. Let $\pi_t^l(x_t) = \bar{u}_t + K_t\delta x_t$ be the linear approximation of the policy. Then, the error in the expected cost to go under the two policies, $|E[J^{\pi}] - E[J^{\pi^l}]|  = O(\epsilon^4)$.
\end{proposition}

Propositions \ref{prop1} and \ref{prop2} form the basis of an $O(\epsilon^2)$ and an $O(\epsilon^4)$ decoupling result in the following subsections.


\subsection{An $O(\epsilon^2)$ Near-Optimal Decoupled Approach for Closed Loop Control} 

%The following observations can now be made from Proposition \ref{prop1}. 
 
%\begin{remark}[Expected cost-to-go]Recall that $u_{t} = \pi_t(x_t)$ $= \bar{u}_t + K_t\delta x_t + \tilde{S}_t(\delta x_t)$. However, note that due to Proposition \ref{prop1}, the expected cost-to-go, $\tilde{J}^{\pi}$, is determined almost solely (within $O(\epsilon^2)$)  by the nominal control action sequence $\bar{u}_t$. In other words, the linear and higher order feedback terms have only $O(\epsilon^2)$ effect on the expected cost-to-go function.
%\end{remark}

%\begin{remark}[Variance of cost-to-go] Given the nominal control action $\bar{u}_t$, the variance of the cost-to-go, which is $O(\epsilon^2)$, is determined overwhelmingly (within $O(\epsilon^4)$) by the linear feedback term $K_t \delta x_t$, i.e., by the variance of the linear perturbation of the cost-to-go, $\delta J_1^{\pi}$, under the linear closed loop system $\delta x_{t+1}^l = (A_t+B_tK_t)\delta x_t^l + \epsilon w_t$.
%\end{remark}
Proposition \ref{prop1} suggests that an open loop control  super imposed with a closed loop control for the perturbed linear system may be approximately optimal. We delineate  this idea below. 

\textit{Open Loop Design.} First, we design an optimal (open loop) control sequence $\bar{u}^{*}_t$ for the noiseless system. More precisely, 
\begin{align}
\label{OL}
(\bar{u}^{*}_t)^{T-1}_{t=1} &= \arg \min_{(\bar{u}_t)^{T-1}_{t=1}} \sum_{t=1}^{T-1} c(\bar{x}_t, \bar{u}_t) + c_T(\bar{x}_T), 
\end{align}%\\
$\bar{x}_{t+1} = f(\bar{x}_t) + g(\bar{x}_{t}) \tilde{u}_t.  
$%\end{align}
We will discuss the details of this open loop design in Section \ref{sec4}. \textit{Albeit non-convex, we can expect to find a global minimum if we can satisfy the necessary conditions for the problem (see the section `Method of Characteristics' in the Supplementary document).}\\
\textit{Closed Loop Design.} We find the optimal feedback gain $K^{*}_t$ such that the variance of the linear closed loop system around the nominal path, $(\bar{x}_t, \bar{u}^{*}_t)$, from the open loop design above, is minimized.  
\begin{align}\label{CL}
(K^{*}_t)^{T-1}_{t=1} &=   \arg \min_{(K_t)^{T-1}_{t=1}} ~ \text{Var}(\delta J_1^{\pi}), 
\end{align}%\nonumber\\
$\delta J_1^{\pi} = \sum_{t=1}^T \bar{C}_t  \delta x_t^l,%\nonumber\\
\delta x_{t+1}^l = (A_t + B_tK_t) \delta x_t^l + \epsilon w_t. $%\label{CL}
%\end{align} 
We now characterize the approximate closed loop policy below. 


\begin{proposition}
\label{propact3}
Construct a closed loop policy 
$\pi_t^*(x_t) = \bar{u}_t^* + K_t^*\delta x_t,$
where $\bar{u}_t^*$ is the solution of the open loop problem \eqref{OL}, and $K_t^*$ is the solution of the closed loop problem \eqref{CL}. Let $\pi^{o}$ be the optimal closed loop policy. Then, 
$| \tilde{J}^{\pi*}  - \tilde{J}^{\pi^o}| = O(\epsilon^2).$
 Furthermore, among all policies with nominal control action $\bar{u}_t^*$, the variance of the cost-to-go under policy $\pi_t^*$, is within $O(\epsilon^4)$ of the variance of the policy with the minimum variance.
 \end{proposition}

%The proof can be found in the supplementary file.

Unfortunately, there is no standard solution to the closed-loop problem \eqref{CL} due to the non additive nature of the cost function $\text{Var}(\delta J_1^{\pi})$. Therefore,  we solve a standard LQR problem as a surrogate, and the effect is again one of reducing the variance of the cost-to-go by reducing the variance of the closed-loop trajectories.

\textit{Approximate Closed Loop Problem.} We solve the following LQR problem for suitably defined cost function weighting factors $Q_t$, $R_t$:

$%$\begin{align}
%\label{eq:acl1}
\min_{(\delta u_t)^{T}_{t=1}} \mathbb{E} [\sum_{t=1}^{T-1} \delta x_t'Q_t\delta x_t+\delta u_t'R_t \delta u_t + \delta x_T'Q_T\delta x_t], \\%\nonumber\\
\delta x_{t+1} = A_t \delta x_t + B_t\delta u_t + \epsilon w_t.
$%\end{align}

The above problem requires the solution of a suitable Ricatti Equation \cite{bryson}, and furnishes us a feedback gain $\hat{K}_t^*$ which we may use in the place of the true variance minimizing gain $K_t^*$.  

%\begin{remark}
%Proposition \ref{prop1} states that the expected cost-to-go of the problem is dominated by the nominal cost-to-go. Therefore, even an open-loop policy consisting of simply the nominal control action is within $O(\epsilon^2)$ of the optimal expected cost-to-go. However, the plan with the optimal feedback gain $K_t^*$ is strictly better than the open-loop plan in that it has a lower variance in terms of the cost to go. Furthermore, solving the approximate closed-loop problem using the surrogate LQR problem, we can expect a lower variance of the cost-to-go function as well.
%which is borne out empirically (albeit we cannot prove it).
%\end{remark}

\subsection{An $O(\epsilon^4)$ Decoupling Result for Closed Loop Control.}
Due to paucity of space, we do not present the $O(\epsilon^4)$ result here, the detailed derivation is provided in the supplementary document. The basic idea is as follows: we show that the performance of the deterministic feedback law when applied to the stochastic system is within $O(\epsilon^4)$ of the (unknown) stochastic optimal law. Next, using Proposition \ref{prop2}, it follows that if we do a linear truncation of the deterministic feedback law, we are within $O(\epsilon^4)$ of its performance, and hence, $O(\epsilon^4)$ of the performance of the optimal stochastic law. Then, we show how to find the linear ( and higher) order terms of the detrministic feedback law using a perturbation analysis of the classical Method of Characteristics (MOC) \cite{Courant-Hilbert}. It suffices to know that while the open loop design is identical, the linear feedback design is changed from the surrogate LQR design in the $O(\epsilon^2)$ design above. 
%In order to derive the results in this section, we need some additional structure on the dynamics. \textit{In essence, the results in this section require that the time discretization of the dynamics be small enough}. Thus, let the dynamics be given by:
%\begin{equation}\label{SDE0}
%x_t = x_{t-1} + \bar{f}(x_{t-1}) \Delta t + \bar{g}(x_{t-1}) u_t \Delta t + \epsilon \omega_t \sqrt{\Delta t},
%\end{equation}
%where $\omega_t$ is a white noise sequence, and the sampling time $\Delta t$ is small enough that $O(\Delta t^{\alpha})$ is negligible for $\alpha > 1$. The noise term above is a Brownian motion, and hence the $\sqrt{\Delta t}$ factor. Further, the incremental cost function $c(x,u)$ is given as:
%$c(x,u) = \bar{l}(x) \Delta t + \frac{1}{2} u'\bar{R}u \Delta t.$
%The main reason to use the above assumptions is to simplify the Dynamic Programming (DP) equation governing the optimal cost-to-go function of the system. The DP equation for the above system is given by:
%\begin{equation}\label{DP}
%J_t(x) = \min_{u_t} \{c(x,u) + E[J_{t+1}(x')]\},
%\end{equation}
%where $x' = x + \bar{f}(x)\Delta t + \bar{g}(x) u_t \Delta t + \epsilon \omega_t \sqrt{\Delta t}$ and $J_t(x)$ denotes the cost-to-go of the system given that it is at state $x$ at time $t$. The above equation is marched back in time with terminal condition $J_T(x) = c_T(x)$, and $c_T(.)$ is the terminal cost function. Let $u_t(.)$ denote the corresponding optimal policy.%Then, it follows that the optimal control $u_t$ satisfies (since the argument to be minimized is quadratic in $u_t$)
%\begin{equation}\label{opt_control}
%u_t= -R^{-1}g' J_{t+1}^x,
%\end{equation}
%where $J_{t+1}^x = \frac{\partial J_{t+1}}{\partial x}$ (see appendix).
 %Further, let $u_t^d(.)$ be the optimal control policy for the deterministic system, i.e., Eq. \ref{SDE0} with $\epsilon =0$. %The optimal cost-to-go of the deterministic system, $\phi_t(.)$ satisfies the deterministic DP equation:
%\begin{equation}\label{detDP}
    %\phi_t(x)= \min_{u}[c(x,u) + \phi_{t+1}(x')],
%\end{equation}
%where $x' = x + f(x')dt + g(x')udt$. Then, identical to the stochastic case, $u_t^d = R^{-1}g'\phi_t^x$.
%Next, let $\varphi_t(.)$ denote the cost-to-go of the deterministic policy when applied to the stochastic system, i.e., $u_t^d$ applied to Eq. \ref{SDE} with $\epsilon > 0$. %The cost-to-go $\varphi_t(.)$ satisfies the policy evaluation equation:
%\begin{equation}\label{detDP_eps}
 %   \varphi_t(x) = c(x, u_t^d(x)) + E[\varphi_{t+1}(x')],
%\end{equation}
%where now $x' = x+ f(x)dt + g(x)u_t^d(x) dt + \epsilon \omega_t \sqrt{dt}$.
%Note the difference between the equations \ref{detDP} and \ref{detDP_eps}.
%Then, we have the following important result.
%\begin{proposition}
%\label{prop_eps}
%The difference between the cost function of the optimal stochastic policy, $J_t$, and the cost function of the ``deterministic policy  applied to the stochastic system", $\varphi_t$, is $O(\epsilon^4)$, i.e. $|J_t (x) - \varphi_t (x)| = O(\epsilon^4)$ for all $(t,x)$.
%\end{proposition}
%The above result was originally proved in a seminal paper \cite{Fleming} for continuous time, first passage problems. We have provided a simple derivation of the result, in the context of a discrete time finite horizon problem, in the Supplementary document. \\

%Given some initial condition $x_0$, consider a linear truncation of the optimal deterministic policy, i.e., let $u_t^l(.) = \bar{u}_t + K_t\delta x_t$, where the deterministic policy is given by $u_t^d = \bar{u}_t + K_t\delta x_t + S_t(\delta x_t)$, where $S_t(.)$ denote the second and higher order terms in the optimal deterministic feedback policy.  Using Proposition \ref{prop2}, it follows that the cost of the linear policy, say $\varphi_t^l(.)$,  is within $O(\epsilon^4)$ of the cost of the deterministic policy $u_t^d(.)$, when applied to the stochastic system in Eq. \ref{SDE0}. However, the result in Proposition \ref{prop_eps} shows that the cost of the deterministic policy is within $O(\epsilon^4)$ of the optimal stochastic policy. Taken together, this implies that the cost of the linear deterministic policy is within $O(\epsilon^4)$ of the optimal stochastic policy. This may be summarized in the following result.
%\begin{proposition} \label{e4}
%Let the optimal cost function under the true stochastic policy be given $J_t(.)$ Let the optimal deterministic policy be given by $u_t^d(x_t) = \bar{u}_t + K_t\delta x_t + S_t(\delta x_t)$, and the linear approximation  to the policy be $u_t^l(x_t) = \bar{u}_t + K_t\delta x_t$, and let the cost of the linear policy be given by $\varphi_t^l(x)$. Then $|J_t(x) - \varphi_t^l(x)| = O(\epsilon^4)$ for all $(t,x)$.
%\end{proposition}

%{\textit{Note : The results provided in this particular section are restated from our prequel paper on D2C primarily for the reader's convenience and for the sake of completeness.}}\\
%In this section, we describe a near-optimal decoupling principle which provides the theoretical foundation for our D2C technique.\\
%Assuming that $f(.)$ and $\pi_t(.)$ are sufficiently smooth, let us describe the linearized dynamics about the nominal trajectory $\mathbb{T}_{nom}$ corresponding to the policy $\pi_t(.)$ as follows. The state and control perturbations, given by $\delta \V{x}_t = \V{x}_t - \bar{\V{x}}_t$ and $\delta \V{u}_t = \V{u}_t - \bar{\V{u}}_t$ respectively, evolve as follows:
%\begin{align}
    %\delta \V{x}_{t+1} &= A_t \delta \V{x}_t + B_t \delta \V{u}_t + S_t(\delta \V{x}_t) + R_t({\delta \V{u}_t}) + \epsilon \omega_t, \label{eq:state_perturbation}
    %\\
    %\delta \V{u}_t &= K_t \delta \V{x}_t + \tilde{S}_t(\delta \V{x}_t) \label{eq:control_perturbation},
%\end{align}
%where $A_t = \frac{\partial f}{\partial {\bf x}}|_{(\bar{\V{x}_t}, \bar{\V{u}}_t)}$, $B_t = \frac{\partial f}{\partial {\bf u}}|_{( \bar{\V{x}}_t,  \bar{\V{u}}_t)}$, $K_t = \frac{\partial \pi(\V{x}_t)}{\partial \V{x}}|_{\bar{\V{x}}_t}$ and $S_t(.)$, $\tilde{S}_t(.)$, $R_t(.)$ are higher order terms in respective Taylor's expansions. 
%By substituting \eqref{eq:control_perturbation} in \eqref{eq:state_perturbation}, we have 
%\begin{align}
 %   \delta \V{x}_{t+1} = \underbrace{(A_t + B_t K_t)}_{\bar{A}_t} \delta \V{x}_t + \bar{S}_t(\delta \V{x}_t) + \epsilon \omega_t,\label{eq:full_state_perturbation}
%\end{align}
%where $\bar{S}_t(\delta \V{x}_t) = B_t \tilde{S}_t (\delta \V{x}_t) + S_t(\delta \V{x}_t) + R_t(K_t\delta \V{x}_t + \tilde{S}_t(\delta \V{x}_t))$. Now, similarly expanding the cost function $c_t(\V{x}_t, \V{u}_t)$ under the policy $ \pi_t(\V{x}_t)$ $\forall t\in\{0,1,\cdots, N-1\}$ about the nominal trajectory $\mathbb{T}_{nom}$ as $c_t(\V{x}_t, \pi_t(\V{x}_t)) = \bar{c}_t + \bar{C}_t \delta \V{x}_t + \bar{H}_t(\delta \V{x}_t)$, where $\bar{c}_t = c_t(\bar{\V{x}}_t, \pi_t(\bar{\V{x}}_t))$ and $\bar{C}_t = \frac{\partial c_t(\V{x}_t, \pi_t(\V{x}_t))}{\partial \V{x}_t}|_{\bar{\V{x}}_t}$ results in
%\begin{equation}
 %   J^{\pi} = \sum_{t=0}^{N} \bar{c}_t + \sum_{t=0}^{N} \bar{C}_t \delta \V{x}_t + \sum_{t=0}^{N} \bar{H}_t(\delta \V{x}_t).
   % \label{eq:cost_to_go_taylors}
%\end{equation}

%{\bf Lemma 1.} The state perturbation equation \eqref{eq:full_state_perturbation} can be equivalently separated into $\delta \V{x}_t = \delta\V{x}_t^l + \bar{S}_t$ and $\delta {\bf x_{t+1}^l} = \bar{A}_t \delta \V{x}_t^l + \epsilon \omega_t$, and $\bar{S}_t$ is $O(\epsilon^2)$.
 
%\vspace{-10pt}
%\begin{proof}
%Proof is provided in the supplementary file under lemma \ref{L1}.
%\end{proof}  
%\vspace{-1pt}
%From \eqref{eq:cost_to_go_taylors} and lemma 1, we obtain
%$
 %   J^{\pi} = \underbrace{\sum_{t=0}^{N} \bar{c}_t}_{\bar{J}^{\pi}} + \underbrace{\sum_{t=0}^{N} \bar{C}_t \delta \V{x}_t^l}_{\delta J^{\pi}_1} + \underbrace{\sum_{t=0}^{N} \bar{H}_t(\delta \V{x}_t) + \bar{C}_t \bar{S}_t}_{\delta J^{\pi}_2}.
%$


%{\bf Proposition 1.} Given a feedback policy $\pi$ satisfying the smoothness requirements,
%\begin{align}
      %  \tilde{J}^{\pi} &= \mathbb{E}[J^{\pi}] = \bar{J}^{\pi} + O(\epsilon^2),\\
       % Var(J^{\pi}) &= \underbrace{Var(\delta J_1^{\pi})}_{O(\epsilon^2)} + O(\epsilon^4).
%\end{align}
%\vspace{-10pt}
%\begin{proof}
%Proof is provided in the supplementary file under Proposition \ref{prop1}.
%\end{proof} 
%\vspace{-10pt}
%Noting that $\V{u}_t = \pi_t(\V{x}_t) = \bar{\V{u}}_t + K_t \delta \V{x}_t + \tilde{S}_t (\delta \V{x}_t)$, the above proposition entails the following observations:\\
%{\bf i) Observation 1:} The cost-to-go along the nominal trajectory $\mathbb{T}_{nom} = \{{\bf \bar{x}_{0:N}}, {\bf \bar{u}_{0:N-1}}\}$ given by $\bar{J}^{\pi}$ is within  $O(\epsilon^2)$ of the expected cost-to-go $\tilde{J}^{\pi}$ of the policy $\pi$.\\
%{\bf ii) Observation 2:} Given the nominal control sequence ${\bf \bar{u}_{0:N-1}}$, the variance of the cost-to-go is overwhelmingly determined by the linear feedback law $K_t \delta \V{x}_t$ $i.e,$ by the variance of the linear perturbation of the cost-to-go, $\delta J_1^{\pi}$, under the linear closed loop system dynamics $\delta \V{x}_{t+1} = \bar{A}_t \delta  \V{x}_t^l + \epsilon \omega_t$.

%Proposition 1 and the above observations suggest that an optimal open-loop control sequence with a suitable linear feedback law (for the perturbed linear system) wrapped around it is approximately optimal. The following subsection summarizes the problems to be solved for each of them.
%\subsection{Decoupled Policy for Feedback Control}
%\label{OL_CL_problems}
%{\bf Open-Loop Trajectory Design:} The open-loop trajectory is designed by solving the noiseless equivalent of the stochastic optimal control problem \eqref{soc_problem},
%$
 %   \underset{\mathbb{T}_{nom}}{\textnormal{min}} \sum^{N-1}_{1} c_t(\bar{\V{x}}_t, \bar{\V{u}}_t) + c_N(\bar{\V{x}_N}), 
    %
  %  ~\textnormal{s.t.}~ \bar{\V{x}}_t = f(\bar{\V{x}}_t, \bar{\V{u}}_t).
%$
%\begin{remark} The open-loop trajectory designed either using model-free ILQR (as shown in section \ref{open_loop_traj_design}) or through gradient descent is the global optimum. The proof (section \ref{MOC} in supplementary material) is based on Method of Characteristics which can be used to get the Lagrange-Charpit equations for the HJB, which when integrated gives a unique characteristic curve of the HJB PDE.
%\end{remark}
%
%{\bf Feedback Law:}
%A linear feedback law is determined by solving for the optimal feedback gains $K_{1:N-1}^*$ that minimize the variance corresponding to the linear perturbation system around the optimal nominal trajectory $\mathbb{T}^*_{nominal}$ found from the above, as follows:
%\begin{align*}
 %   \underset{\{K_{1:N-1}\}}{\textnormal{min}}~ &Var(\delta J_1^{\pi}),
%\end{align*}
%where,    
%$
%\delta J_1^{\pi} = \sum_{t=1}^{N} \bar{C}_t \delta \V{x}_t^l
%$
%and
%$
%    \delta \V{x}_{t+1} = (A_t + B_t K_t)\delta \V{x}_t^l + \epsilon \omega_t.
%$

%Albeit convex, the above problem does not have a standard solution. However, since we are really only interested in a good variance rather than the optimal variance, we can solve an inexpensive  time-varying LQR problem as a surrogate to reduce the variance of the cost-to-go. The corresponding problem can be posed as follows:
%$
 %   \underset{{\delta {\bf u_{1:N}}}}{\textnormal{min}}~ \mathbb{E}[\sum_{t=1}^{N-1} \delta \V{x}_t^T Q_t \delta \V{x}_t + \delta \V{u}_t^T R_t \delta \V{u}_t + \delta \V{x}_N^T Q_N \delta \V{x}_N],
    %
  %  \textnormal{s.t.}~\delta \V{x}_{t+1} = A_t \delta \V{x}_t + B_t \V{u}_t + \epsilon \omega_t. 
%$
%\begin{remark}
%In fact, if the feedback gain is designed carefully rather than the heuristic LQR above, then one can obtain $O(\epsilon^4)$ near-optimality. The proof is shown in the supplementary document under section \ref{Oe4}.
%\end{remark}

==> Related_work.tex <==
\section{Related Work}
\label{related_work}
% \vspace{-10pt}
Differential Dynamic Programming (DDP) \cite{mayne's ddp} is a class of iterative algorithms for trajectory optimization. One salient aspect of DDP is that it exhibits quadratic convergence for a general non-linear optimal control problem and can be solved in a single step for linear systems. In spite of its origins in the 1960s, it gained popularity only in the last decade due to the success of the modified algorithm called ILQR \cite{ilqr-1}. Though DDP (theoretically) guarantees a quadratic convergence, some of the terms in it involve computing second-order derivatives of the system dynamical models. Since the dynamical models of most systems are multivariable vector-valued functions and their second-order derivatives being third-order tensors, DDP in its original form was not effective for practical implementation. ILQR \cite{ilqr} \cite{ILQG} dropped these terms and introduced regularization schemes \cite{ddp with nonlinear constraints}\cite{ILQG_complex_behaviors} to handle the absence of these computationally expensive terms. This resulted in a faster and more stable convergence to the optimal solution.

One advantage that ILQR has in terms of solving it in a model-free manner is that this algorithm is explicit in terms of system model and their first-order derivatives. Earlier works such as by \cite{ILQG_complex_behaviors} and \cite{Levine} employed finite differencing in computing the Jacobians in ILQR. Typically, a forward Euler scheme is chosen to independently determine each element ({\it i.e,} gradient) in a Jacobian matrix.  \cite{Mitrovic2010} presented ILQR-LD by learning the dynamics through Locally Weighted Projection Regression (LWPR) approximation of the model first and then obtaining a corresponding analytical Jacobian. Their work also demonstrated better computational efficiency over finite differences.

Spall introduced the `Simultaneous Perturbation Stochastic Approximation' (SPSA) \cite{spsa} method that evaluates the function only twice to calculate the Jacobian of the cost function. In this paper, a similar formulation is derived to compute the Jacobians of the system model online, in a model-free fashion, through the least squares method in a central-difference scheme.

The rest of the paper is organized as follows. Section \ref{problem_formulation} introduces the terminology and provides the problem statement. In section \ref{decoupling_principle}, we present a near-optimal decoupling principle that forms the basis of our algorithm. Section \ref{algorithm} describes our algorithm - D2C 2.0 in detail. In Sections \ref{simulations} and \ref{discussion}, we provide results and a discussion of the application of the D2C 2.0 to several benchmark examples, along with comparisons to DDPG and the D2C technique.
